EdgeRAG: Online-Indexed RAG for Edge Devices

Deploying Retrieval Augmented Generation (RAG) on resource-constrained edge devices is challenging due to limited memory and processing power. In this work, we propose EdgeRAG which addresses the memory constraint by pruning embeddings within clusters and generating embeddings on-demand during retrieval. To avoid the latency of generating embeddings for large tail clusters, EdgeRAG pre-computes and stores embeddings for these clusters, while adaptively caching remaining embeddings to minimize redundant computations and further optimize latency. The result from BEIR suite shows that EdgeRAG offers significant latency reduction over the baseline IVF index, but with similar generation quality while allowing all of our evaluated datasets to fit into the memory.

==> not_used/permeable.tex <==
%%%%%%%%%%%%%% Packages %%%%%%%%%%%%%%

\usepackage{mathptmx} % This is Times font
\usepackage[sort, compress]{cite}
\renewcommand\citepunct{, }
\usepackage{subcaption}
\usepackage{overpic}
\usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{booktabs} % for professional tables
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{fancyhdr}
\usepackage[normalem]{ulem}
% \usepackage{microtype}
\usepackage{xspace}
\usepackage{adjustbox}
\usepackage{array}
\usepackage{pifont}
%\usepackage{subfig}
%\usepackage[justification=centering]{caption}
%\usepackage{graphicx}
%\usepackage[justification=centering]{subcaption}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{hhline}
\usepackage{etoolbox}
\usepackage{comment}
\usepackage{tipa}
\usepackage{dblfloatfix} 
% Ensure letter paper
% \pdfpagewidth=8.5in
% \pdfpageheight=11in
\usepackage{booktabs}
% Always include hyperref last
\usepackage{url}
% Break long URL
% \makeatletter
% \g@addto@macro{\UrlBreaks}{\UrlOrds}
% \makeatother
% \usepackage[anythingbreaks]{breakurl}
\usepackage[colorlinks=true,citecolor=blue]{hyperref}
\usepackage{enumitem}
\usepackage{wrapfig}
\usepackage{balance}
\usepackage{xcolor}

%%%%%%%%%%%%%% New Commands %%%%%%%%%%%%%%

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }
    
\newcommand{\ignore}[1]{}

\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}


\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


% Ensure letter paper
\pdfpagewidth=8.5in
\pdfpageheight=11in

==> old_style/permeable.tex <==
%%%%%%%%%%%%%% Packages %%%%%%%%%%%%%%

% \usepackage{mathptmx} % This is Times font
\usepackage[sort, compress]{cite}
% \renewcommand\citepunct{, }
% \usepackage{authblk}
\usepackage{subcaption}
%\usepackage{subfigure}
\usepackage{overpic}

\usepackage{mathptmx} % This is Times font
\usepackage{amsmath}% http://ctan.org/pkg/amsmath
% \usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{fancyhdr}
\usepackage[normalem]{ulem}
\usepackage{microtype}
\usepackage{xspace}
\usepackage{adjustbox}
\usepackage{array}
\usepackage{pifont}
%\usepackage{subfig}
%\usepackage[justification=centering]{caption}
%\usepackage{graphicx}
%\usepackage[justification=centering]{subcaption}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{hhline}
\usepackage{etoolbox}
\usepackage{comment}
\usepackage{tipa}
\usepackage{dblfloatfix} 
% Ensure letter paper
% \pdfpagewidth=8.5in
% \pdfpageheight=11in
\usepackage{booktabs}
% Always include hyperref last
% \usepackage[colorlinks=true,citecolor=blue]{hyperref}
%\usepackage[hyphens]{url}

%%%%%%%%%%%%%% New Commands %%%%%%%%%%%%%%

\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }
    
\newcommand{\ignore}[1]{}

\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}


==> tab/comparison.tex <==

\begin{table*}[h]
\centering
% \small
\setlength{\tabcolsep}{1pt}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
 \multicolumn{1}{|c|}{\textbf{Design Choices}} & 
 \multicolumn{1}{c|}{\textbf{Log Location}} & 
 \multicolumn{1}{c|}{\textbf{Log Latency}} &
 \multicolumn{1}{C{2.5cm}|}{\textbf{Request Latency (No replication)}} &
 \multicolumn{1}{C{2.5cm}|}{\textbf{Request Latency (3-way replication)}} & 
 \multicolumn{1}{c|}{\textbf{Hardware Reconfiguration}} \\
%  \multicolumn{1}{c|}{\textbf{Replication Latency}} \\
    \hline
    {Client-sided Logging\cite{arteaga2014client, kim2015request, qin2014reliable, liao2005collective}} & {Client} & {$\sim 5$ us} & {$<$ 10 us} & {$\sim 50$ us} & {PM in all clients}   \\
    \hline
    %{Dedicated Logging hosts} & {Logging host} & {High} & {$<$ 81 Gbps} & {Additional Server with PM}  \\
    %\hline
    {Server-sided logging\cite{ghandeharizadeh2019design}} & {Server} & {$\sim 5$ us} & {$\sim 40$ us} & {$\sim 80$ us} & {PM in all servers}    \\
    \hline
    {\textbf{\xname{}} (this work)} & {Switch or NIC} & {$\sim 1$ us} & {$\sim 20$ us} & {$\sim 22$ us} & {Switch/NIC with PM}   \\
    \hline
\end{tabular}
\caption{A comparison among alternative request-logging implementations (200-Byte request payload).}
% \todo{add read cache?, range of latency instead of high-low, BW, where does number come from: address in the text, cite the setup}} 
\label{tab:pmnet_alts}
\vspace{-2em}
\end{table*}


==> tab/dataset_compare.tex <==
\begin{table}
%\vspace{-0.5em}
\setlength{\tabcolsep}{1pt}
\footnotesize
    \centering
    \caption{Dataset size comparision}
    % \vspace{-0.05in}
    \begin{tabular}{l|l|l|l}
       \toprule
    %   \multicolumn{1}{|c|}{\textbf{Function}} & \multicolumn{1}{c|}{\textbf{Description}} \\
    %   \hline
       % Client
       Dataset & Corpus & Records & Embedding \\
       \hline
       scidocs \cite{specter2020cohan} & 86 M & 3.6 k & 113 MB \\
       fiqa \cite{www18}& 130 MB & 25 k & 217 MB \\
       quora \cite{Quora}& 641 MB & 523 k & 1.5 GB \\
       nq \cite{kwiatkowski-etal-2019-natural}& 4.6 GB & 2.68 M & 8.3 GB \\
       hotpotqa \cite{thorne-etal-2018-fever}& 11 GB & 5.42 M & 15.4 GB \\
       fever \cite{yang-etal-2018-hotpotqa}& 7.5 GB & 5.23 M & 18.5 GB \\
       \bottomrule
    \end{tabular}
    \label{tab:datasets}
    % \vspace{-0.1in}
\end{table}
